$\tau$ lepton mass measurement at Belle II

The reconstruction of tau-pair production, $e^{+}e^{-} \to \tau^{+}\tau^{-}$, from the subsequent 3-prong ($\tau^{+} \rightarrow \pi^{+} \pi^{-} \pi^{+} \bar{\nu}_{\tau}$) and 1-prong ($\tau^{-} \to \ell^{-} \bar{\nu}_{\ell} \nu_{\tau}$, $\tau^{-} \to h^{-} \nu_{\tau}$ or $\tau^{-} \to \pi^{-} \pi^0 \nu_{\tau}$) decays, is presented using 8.8 fb$^{-1}$ of $e^{+}e^{-}$ collision data of Belle II at the center-of-mass energy $\sqrt{s} = m_{\Upsilon(4S)}$. The pseudomass technique developed by the ARGUS experiment is used to measure the $\tau$-lepton mass $m_{\tau}$ in the 3-prong $\tau^{+} \to \pi^{+} \pi^{-} \pi^{+} \bar{\nu}_{\tau} $ decay, resulting in $m_{\tau} = 1777.28 \pm 0.75~{\rm (stat.)} \pm 0.33 ~{\rm (sys.)}~{\rm{MeV}/\rm{c}^2}$.

==> addref <==
#!/usr/bin/env python3
# -*- coding: utf-8 -*-

from urllib.request import urlopen
import sys
import re

# check arguments
if len(sys.argv) != 2:
    print('ERROR: An arXiv or inspire ID has to be given as argument')
    sys.exit(1)

id = sys.argv[1]
bibfile = 'references.bib'

# convert arxiv to inspire ID
if '/' in id or '.' in id:
    if ':' in id:
        id = id[id.find(':')+1:]
    data = urlopen(f'http://inspirehep.net/search?p=find+eprint+{id}').read()
    match = re.compile(b'record/(\d*)').findall(data)
    if not match:
        print(f'ERROR: Could not get inspire ID for arXiv number {id}.')
        sys.exit(1)
    id = match[0].decode()

# get bibtex from inspire
data = urlopen(f'http://inspirehep.net/record/{id}/export/hx').read()
match = re.compile(b'[\S\s]*<pre>\n([\S\s]*)</pre>[\S\s]*').findall(data)
if not match:
    print(f'ERROR: Could not get bibtex for inspire ID {id}.')
    sys.exit(1)
bibtex = match[0].decode()

# check whether the entry is already in references.bib
entry = re.compile('@[\w]*{([\S]*),').findall(bibtex)[0]
with open(bibfile) as bib:
    if entry in bib.read():
        print(f'ERROR: {bibfile} already contains the entry {entry}.')
        sys.exit(1)

# add bibtex to references.bib
with open(bibfile, 'a+') as bib:
    bib.write('\n' + bibtex)

print(f'Entry {entry} added to {bibfile} -> \\cite{{{entry}}}')

==> authors.tex <==
%%% Paper:    (2020  conference papers)
%%% Journal:  (2020 conferences)
%%% ====================================================================
%%% Use \input{authors-conf2020} to insert this material into your latex file.
\newcommand{\instSinica}{Academia Sinica, Taipei 11529, Taiwan}
\newcommand{\instCPPM}{Aix Marseille Universit\'{e}, CNRS/IN2P3, CPPM, 13288 Marseille, France}
\newcommand{\instBeihang}{Beihang University, Beijing 100191, China}
\newcommand{\instBUAP}{Benemerita Universidad Autonoma de Puebla, Puebla 72570, Mexico}
\newcommand{\instBNL}{Brookhaven National Laboratory, Upton, New York 11973, U.S.A.}
\newcommand{\instBINP}{Budker Institute of Nuclear Physics SB RAS, Novosibirsk 630090, Russian Federation}
\newcommand{\instCMU}{Carnegie Mellon University, Pittsburgh, Pennsylvania 15213, U.S.A.}
\newcommand{\instCinvestavIPN}{Centro de Investigacion y de Estudios Avanzados del Instituto Politecnico Nacional, Mexico City 07360, Mexico}
\newcommand{\instPrague}{Faculty of Mathematics and Physics, Charles University, 121 16 Prague, Czech Republic}
\newcommand{\instChiangMai}{Chiang Mai University, Chiang Mai 50202, Thailand}
\newcommand{\instChiba}{Chiba University, Chiba 263-8522, Japan}
\newcommand{\instChonnam}{Chonnam National University, Gwangju 61186, South Korea}
\newcommand{\instConacyt}{Consejo Nacional de Ciencia y Tecnolog\'{\i}a, Mexico City 03940, Mexico}
\newcommand{\instDESY}{Deutsches Elektronen--Synchrotron, 22607 Hamburg, Germany}
\newcommand{\instDuke}{Duke University, Durham, North Carolina 27708, U.S.A.}
\newcommand{\instITAR}{Institute of Theoretical and Applied Research (ITAR), Duy Tan University, Hanoi 100000, Vietnam}
\newcommand{\instENEA}{ENEA Casaccia, I-00123 Roma, Italy}
\newcommand{\instEri}{Earthquake Research Institute, University of Tokyo, Tokyo 113-0032, Japan}
\newcommand{\instJuelich}{Forschungszentrum J\"{u}lich, 52425 J\"{u}lich, Germany}
\newcommand{\instFuJen}{Department of Physics, Fu Jen Catholic University, Taipei 24205, Taiwan}
\newcommand{\instFudan}{Key Laboratory of Nuclear Physics and Ion-beam Application (MOE) and Institute of Modern Physics, Fudan University, Shanghai 200443, China}
\newcommand{\instGoettingen}{II. Physikalisches Institut, Georg-August-Universit\"{a}t G\"{o}ttingen, 37073 G\"{o}ttingen, Germany}
\newcommand{\instGifu}{Gifu University, Gifu 501-1193, Japan}
\newcommand{\instSOKENDAI}{The Graduate University for Advanced Studies (SOKENDAI), Hayama 240-0193, Japan}
\newcommand{\instGyeongsang}{Gyeongsang National University, Jinju 52828, South Korea}
\newcommand{\instHanyang}{Department of Physics and Institute of Natural Sciences, Hanyang University, Seoul 04763, South Korea}
\newcommand{\instKEK}{High Energy Accelerator Research Organization (KEK), Tsukuba 305-0801, Japan}
\newcommand{\instJPARC}{J-PARC Branch, KEK Theory Center, High Energy Accelerator Research Organization (KEK), Tsukuba 305-0801, Japan}
\newcommand{\instHSE}{Higher School of Economics (HSE), Moscow 101000, Russian Federation}
\newcommand{\instIISER}{Indian Institute of Science Education and Research Mohali, SAS Nagar, 140306, India}
\newcommand{\instIITBhubaneswar}{Indian Institute of Technology Bhubaneswar, Satya Nagar 751007, India}
\newcommand{\instIITGuwahati}{Indian Institute of Technology Guwahati, Assam 781039, India}
\newcommand{\instIITHyderabad}{Indian Institute of Technology Hyderabad, Telangana 502285, India}
\newcommand{\instIITMadras}{Indian Institute of Technology Madras, Chennai 600036, India}
\newcommand{\instIndiana}{Indiana University, Bloomington, Indiana 47408, U.S.A.}
\newcommand{\instIHEPRussia}{Institute for High Energy Physics, Protvino 142281, Russian Federation}
\newcommand{\instHEPHYVienna}{Institute of High Energy Physics, Vienna 1050, Austria}
\newcommand{\instIHEPChina}{Institute of High Energy Physics, Chinese Academy of Sciences, Beijing 100049, China}
\newcommand{\instChennai}{Institute of Mathematical Sciences, Chennai 600113, India}
\newcommand{\instIPP}{Institute of Particle Physics (Canada), Victoria, British Columbia V8W 2Y2, Canada}
\newcommand{\instIOP}{Institute of Physics, Vietnam Academy of Science and Technology (VAST), Hanoi, Vietnam}
\newcommand{\instIFIC}{Instituto de Fisica Corpuscular, Paterna 46980, Spain}
\newcommand{\instFrascati}{INFN Laboratori Nazionali di Frascati, I-00044 Frascati, Italy}
\newcommand{\instNapoliINFN}{INFN Sezione di Napoli, I-80126 Napoli, Italy}
\newcommand{\instPadovaINFN}{INFN Sezione di Padova, I-35131 Padova, Italy}
\newcommand{\instPerugiaINFN}{INFN Sezione di Perugia, I-06123 Perugia, Italy}
\newcommand{\instPisaINFN}{INFN Sezione di Pisa, I-56127 Pisa, Italy}
\newcommand{\instRomaINFN}{INFN Sezione di Roma, I-00185 Roma, Italy}
\newcommand{\instRomaTreINFN}{INFN Sezione di Roma Tre, I-00146 Roma, Italy}
\newcommand{\instTorinoINFN}{INFN Sezione di Torino, I-10125 Torino, Italy}
\newcommand{\instTriesteINFN}{INFN Sezione di Trieste, I-34127 Trieste, Italy}
\newcommand{\instJAEA}{Advanced Science Research Center, Japan Atomic Energy Agency, Naka 319-1195, Japan}
\newcommand{\instMainz}{Johannes Gutenberg-Universit\"{a}t Mainz, Institut f\"{u}r Kernphysik, D-55099 Mainz, Germany}
\newcommand{\instGiessen}{Justus-Liebig-Universit\"{a}t Gie\ss{}en, 35392 Gie\ss{}en, Germany}
\newcommand{\instKarlsruhe}{Institut f\"{u}r Experimentelle Teilchenphysik, Karlsruher Institut f\"{u}r Technologie, 76131 Karlsruhe, Germany}
\newcommand{\instKennesaw}{Kennesaw State University, Kennesaw, Georgia 30144, U.S.A.}
\newcommand{\instKitasato}{Kitasato University, Sagamihara 252-0373, Japan}
\newcommand{\instKISTI}{Korea Institute of Science and Technology Information, Daejeon 34141, South Korea}
\newcommand{\instKorea}{Korea University, Seoul 02841, South Korea}
\newcommand{\instKSU}{Kyoto Sangyo University, Kyoto 603-8555, Japan}
\newcommand{\instKyotoU}{Kyoto University, Kyoto 606-8501, Japan}
\newcommand{\instKyungpook}{Kyungpook National University, Daegu 41566, South Korea}
\newcommand{\instLPI}{P.N. Lebedev Physical Institute of the Russian Academy of Sciences, Moscow 119991, Russian Federation}
\newcommand{\instLNNU}{Liaoning Normal University, Dalian 116029, China}
\newcommand{\instLMU}{Ludwig Maximilians University, 80539 Munich, Germany}
\newcommand{\instLuther}{Luther College, Decorah, Iowa 52101, U.S.A.}
\newcommand{\instMNITJaipur}{Malaviya National Institute of Technology Jaipur, Jaipur 302017, India}
\newcommand{\instMPP}{Max-Planck-Institut f\"{u}r Physik, 80805 M\"{u}nchen, Germany}
\newcommand{\instMPGHLL}{Semiconductor Laboratory of the Max Planck Society, 81739 M\"{u}nchen, Germany}
\newcommand{\instMcGill}{McGill University, Montr\'{e}al, Qu\'{e}bec, H3A 2T8, Canada}
\newcommand{\instMETU}{Middle East Technical University, 06531 Ankara, Turkey}
\newcommand{\instMEPhI}{Moscow Physical Engineering Institute, Moscow 115409, Russian Federation}
\newcommand{\instNagoya}{Graduate School of Science, Nagoya University, Nagoya 464-8602, Japan}
\newcommand{\instNagoyaKMI}{Kobayashi-Maskawa Institute, Nagoya University, Nagoya 464-8602, Japan}
\newcommand{\instNagoyaIAR}{Institute for Advanced Research, Nagoya University, Nagoya 464-8602, Japan}
\newcommand{\instNaraWu}{Nara Women's University, Nara 630-8506, Japan}
\newcommand{\instUNAM}{National Autonomous University of Mexico, Mexico City, Mexico}
\newcommand{\instNTUTaiwan}{Department of Physics, National Taiwan University, Taipei 10617, Taiwan}
\newcommand{\instNUUTaiwan}{National United University, Miao Li 36003, Taiwan}
\newcommand{\instKrakow}{H. Niewodniczanski Institute of Nuclear Physics, Krakow 31-342, Poland}
\newcommand{\instNiigata}{Niigata University, Niigata 950-2181, Japan}
\newcommand{\instNSU}{Novosibirsk State University, Novosibirsk 630090, Russian Federation}
\newcommand{\instOkinawa}{Okinawa Institute of Science and Technology, Okinawa 904-0495, Japan}
\newcommand{\instOsakaCity}{Osaka City University, Osaka 558-8585, Japan}
\newcommand{\instRCNP}{Research Center for Nuclear Physics, Osaka University, Osaka 567-0047, Japan}
\newcommand{\instPNNL}{Pacific Northwest National Laboratory, Richland, Washington 99352, U.S.A.}
\newcommand{\instPanjab}{Panjab University, Chandigarh 160014, India}
\newcommand{\instPeking}{Peking University, Beijing 100871, China}
\newcommand{\instPanjabPAU}{Punjab Agricultural University, Ludhiana 141004, India}
\newcommand{\instRIKENMSL}{Meson Science Laboratory, Cluster for Pioneering Research, RIKEN, Saitama 351-0198, Japan}
\newcommand{\instRIKEN}{Theoretical Research Division, Nishina Center, RIKEN, Saitama 351-0198, Japan}
\newcommand{\instXavier}{St. Francis Xavier University, Antigonish, Nova Scotia, B2G 2W5, Canada}
\newcommand{\instSeoul}{Seoul National University, Seoul 08826, South Korea}
\newcommand{\instShandong}{Shandong University, Jinan 250100, China}
\newcommand{\instSPU}{Showa Pharmaceutical University, Tokyo 194-8543, Japan}
\newcommand{\instSoochow}{Soochow University, Suzhou 215006, China}
\newcommand{\instSoongsil}{Soongsil University, Seoul 06978, South Korea}
\newcommand{\instLjubljanaJSI}{J. Stefan Institute, 1000 Ljubljana, Slovenia}
\newcommand{\instKyiv}{Taras Shevchenko National Univ. of Kiev, Kiev, Ukraine}
\newcommand{\instTata}{Tata Institute of Fundamental Research, Mumbai 400005, India}
\newcommand{\instTUM}{Department of Physics, Technische Universit\"{a}t M\"{u}nchen, 85748 Garching, Germany}
\newcommand{\instECUTUM}{Excellence Cluster Universe, Technische Universit\"{a}t M\"{u}nchen, 85748 Garching, Germany}
\newcommand{\instTelAviv}{Tel Aviv University, School of Physics and Astronomy, Tel Aviv, 69978, Israel}
\newcommand{\instToho}{Toho University, Funabashi 274-8510, Japan}
\newcommand{\instTohoku}{Department of Physics, Tohoku University, Sendai 980-8578, Japan}
\newcommand{\instTitech}{Tokyo Institute of Technology, Tokyo 152-8550, Japan}
\newcommand{\instTokyoMetropolitan}{Tokyo Metropolitan University, Tokyo 192-0397, Japan}
\newcommand{\instUAS}{Universidad Autonoma de Sinaloa, Sinaloa 80000, Mexico}
\newcommand{\instNapoliUNIV}{Dipartimento di Scienze Fisiche, Universit\`{a} di Napoli Federico II, I-80126 Napoli, Italy}
\newcommand{\instNapoliUNIVA}{Dipartimento di Agraria, Universit\`{a} di Napoli Federico II, I-80055 Portici (NA), Italy}
\newcommand{\instPadovaUNIV}{Dipartimento di Fisica e Astronomia, Universit\`{a} di Padova, I-35131 Padova, Italy}
\newcommand{\instPerugiaUNIV}{Dipartimento di Fisica, Universit\`{a} di Perugia, I-06123 Perugia, Italy}
\newcommand{\instPisaUNIV}{Dipartimento di Fisica, Universit\`{a} di Pisa, I-56127 Pisa, Italy}
\newcommand{\instRomaUNIV}{Universit\`{a} di Roma ``La Sapienza,'' I-00185 Roma, Italy}
\newcommand{\instRomaTreUNIV}{Dipartimento di Matematica e Fisica, Universit\`{a} di Roma Tre, I-00146 Roma, Italy}
\newcommand{\instTorinoUNIV}{Dipartimento di Fisica, Universit\`{a} di Torino, I-10125 Torino, Italy}
\newcommand{\instTriesteUNIV}{Dipartimento di Fisica, Universit\`{a} di Trieste, I-34127 Trieste, Italy}
\newcommand{\instMontreal}{Universit\'{e} de Montr\'{e}al, Physique des Particules, Montr\'{e}al, Qu\'{e}bec, H3C 3J7, Canada}
\newcommand{\instIJCLab}{Universit\'{e} Paris-Saclay, CNRS/IN2P3, IJCLab, 91405 Orsay, France}
\newcommand{\instIPHC}{Universit\'{e} de Strasbourg, CNRS, IPHC, UMR 7178, 67037 Strasbourg, France}
\newcommand{\instAdelaide}{Department of Physics, University of Adelaide, Adelaide, South Australia 5005, Australia}
\newcommand{\instBonn}{University of Bonn, 53115 Bonn, Germany}
\newcommand{\instUBC}{University of British Columbia, Vancouver, British Columbia, V6T 1Z1, Canada}
\newcommand{\instCincinnati}{University of Cincinnati, Cincinnati, Ohio 45221, U.S.A.}
\newcommand{\instFlorida}{University of Florida, Gainesville, Florida 32611, U.S.A.}
\newcommand{\instHamburg}{University of Hamburg, 20148 Hamburg, Germany}
\newcommand{\instHawaii}{University of Hawaii, Honolulu, Hawaii 96822, U.S.A.}
\newcommand{\instHeidelberg}{University of Heidelberg, 68131 Mannheim, Germany}
\newcommand{\instLjubljanaUniLJ}{Faculty of Mathematics and Physics, University of Ljubljana, 1000 Ljubljana, Slovenia}
\newcommand{\instLouisville}{University of Louisville, Louisville, Kentucky 40292, U.S.A.}
\newcommand{\instMalaya}{National Centre for Particle Physics, University Malaya, 50603 Kuala Lumpur, Malaysia}
\newcommand{\instLjubljanaUM}{University of Maribor, 2000 Maribor, Slovenia}
\newcommand{\instMelbourne}{School of Physics, University of Melbourne, Victoria 3010, Australia}
\newcommand{\instMississippi}{University of Mississippi, University, Mississippi 38677, U.S.A.}
\newcommand{\instUOM}{University of Miyazaki, Miyazaki 889-2192, Japan}
\newcommand{\instNovaGorica}{University of Nova Gorica, 5000 Nova Gorica, Slovenia}
\newcommand{\instPittsburgh}{University of Pittsburgh, Pittsburgh, Pennsylvania 15260, U.S.A.}
\newcommand{\instUSTC}{University of Science and Technology of China, Hefei 230026, China}
\newcommand{\instSAlabama}{University of South Alabama, Mobile, Alabama 36688, U.S.A.}
\newcommand{\instSCarolina}{University of South Carolina, Columbia, South Carolina 29208, U.S.A.}
\newcommand{\instSydney}{School of Physics, University of Sydney, New South Wales 2006, Australia}
\newcommand{\instTabuk}{Department of Physics, Faculty of Science, University of Tabuk, Tabuk 71451, Saudi Arabia}
\newcommand{\instUTokyo}{Department of Physics, University of Tokyo, Tokyo 113-0033, Japan}
\newcommand{\instIPMU}{Kavli Institute for the Physics and Mathematics of the Universe (WPI), University of Tokyo, Kashiwa 277-8583, Japan}
\newcommand{\instVictoria}{University of Victoria, Victoria, British Columbia, V8W 3P6, Canada}
\newcommand{\instVPI}{Virginia Polytechnic Institute and State University, Blacksburg, Virginia 24061, U.S.A.}
\newcommand{\instWayneState}{Wayne State University, Detroit, Michigan 48202, U.S.A.}
\newcommand{\instYamagata}{Yamagata University, Yamagata 990-8560, Japan}
\newcommand{\instYerevan}{Alikhanyan National Science Laboratory, Yerevan 0036, Armenia}
\newcommand{\instYonsei}{Yonsei University, Seoul 03722, South Korea}
%%%\affiliation{\instSinica}
\affiliation{\instCPPM}
\affiliation{\instBeihang}
%%%\affiliation{\instBUAP}
\affiliation{\instBNL}
\affiliation{\instBINP}
\affiliation{\instCMU}
\affiliation{\instCinvestavIPN}
\affiliation{\instPrague}
\affiliation{\instChiangMai}
\affiliation{\instChiba}
\affiliation{\instChonnam}
\affiliation{\instConacyt}
\affiliation{\instDESY}
\affiliation{\instDuke}
\affiliation{\instITAR}
%%%\affiliation{\instENEA}
\affiliation{\instEri}
\affiliation{\instJuelich}
\affiliation{\instFuJen}
\affiliation{\instFudan}
\affiliation{\instGoettingen}
\affiliation{\instGifu}
\affiliation{\instSOKENDAI}
\affiliation{\instGyeongsang}
\affiliation{\instHanyang}
\affiliation{\instKEK}
\affiliation{\instJPARC}
\affiliation{\instHSE}
\affiliation{\instIISER}
\affiliation{\instIITBhubaneswar}
\affiliation{\instIITGuwahati}
\affiliation{\instIITHyderabad}
\affiliation{\instIITMadras}
\affiliation{\instIndiana}
\affiliation{\instIHEPRussia}
\affiliation{\instHEPHYVienna}
\affiliation{\instIHEPChina}
%%%\affiliation{\instChennai}
\affiliation{\instIPP}
\affiliation{\instIOP}
\affiliation{\instIFIC}
\affiliation{\instFrascati}
\affiliation{\instNapoliINFN}
\affiliation{\instPadovaINFN}
\affiliation{\instPerugiaINFN}
\affiliation{\instPisaINFN}
\affiliation{\instRomaINFN}
\affiliation{\instRomaTreINFN}
\affiliation{\instTorinoINFN}
\affiliation{\instTriesteINFN}
\affiliation{\instJAEA}
\affiliation{\instMainz}
\affiliation{\instGiessen}
\affiliation{\instKarlsruhe}
%%%\affiliation{\instKennesaw}
\affiliation{\instKitasato}
\affiliation{\instKISTI}
\affiliation{\instKorea}
\affiliation{\instKSU}
%%%\affiliation{\instKyotoU}
\affiliation{\instKyungpook}
\affiliation{\instLPI}
\affiliation{\instLNNU}
\affiliation{\instLMU}
\affiliation{\instLuther}
\affiliation{\instMNITJaipur}
\affiliation{\instMPP}
\affiliation{\instMPGHLL}
\affiliation{\instMcGill}
%%%\affiliation{\instMETU}
\affiliation{\instMEPhI}
\affiliation{\instNagoya}
\affiliation{\instNagoyaKMI}
\affiliation{\instNagoyaIAR}
\affiliation{\instNaraWu}
%%%\affiliation{\instUNAM}
\affiliation{\instNTUTaiwan}
\affiliation{\instNUUTaiwan}
\affiliation{\instKrakow}
\affiliation{\instNiigata}
\affiliation{\instNSU}
\affiliation{\instOkinawa}
\affiliation{\instOsakaCity}
\affiliation{\instRCNP}
\affiliation{\instPNNL}
\affiliation{\instPanjab}
\affiliation{\instPeking}
\affiliation{\instPanjabPAU}
\affiliation{\instRIKENMSL}
%%%\affiliation{\instRIKEN}
%%%\affiliation{\instXavier}
\affiliation{\instSeoul}
%%%\affiliation{\instShandong}
\affiliation{\instSPU}
\affiliation{\instSoochow}
\affiliation{\instSoongsil}
\affiliation{\instLjubljanaJSI}
\affiliation{\instKyiv}
\affiliation{\instTata}
\affiliation{\instTUM}
%%%\affiliation{\instECUTUM}
\affiliation{\instTelAviv}
\affiliation{\instToho}
\affiliation{\instTohoku}
\affiliation{\instTitech}
\affiliation{\instTokyoMetropolitan}
\affiliation{\instUAS}
\affiliation{\instNapoliUNIV}
\affiliation{\instPadovaUNIV}
\affiliation{\instPerugiaUNIV}
\affiliation{\instPisaUNIV}
\affiliation{\instRomaUNIV}
\affiliation{\instRomaTreUNIV}
\affiliation{\instTorinoUNIV}
\affiliation{\instTriesteUNIV}
\affiliation{\instMontreal}
\affiliation{\instIJCLab}
\affiliation{\instIPHC}
\affiliation{\instAdelaide}
\affiliation{\instBonn}
\affiliation{\instUBC}
\affiliation{\instCincinnati}
\affiliation{\instFlorida}
%%%\affiliation{\instHamburg}
\affiliation{\instHawaii}
\affiliation{\instHeidelberg}
\affiliation{\instLjubljanaUniLJ}
\affiliation{\instLouisville}
\affiliation{\instMalaya}
\affiliation{\instLjubljanaUM}
\affiliation{\instMelbourne}
\affiliation{\instMississippi}
\affiliation{\instUOM}
%%%\affiliation{\instNovaGorica}
\affiliation{\instPittsburgh}
\affiliation{\instUSTC}
\affiliation{\instSAlabama}
\affiliation{\instSCarolina}
\affiliation{\instSydney}
%%%\affiliation{\instTabuk}
\affiliation{\instUTokyo}
\affiliation{\instIPMU}
\affiliation{\instVictoria}
\affiliation{\instVPI}
\affiliation{\instWayneState}
\affiliation{\instYamagata}
\affiliation{\instYerevan}
\affiliation{\instYonsei}
  \author{F.~Abudin{\'e}n}\affiliation{\instTriesteINFN} % 2250
  \author{I.~Adachi}\affiliation{\instKEK}\affiliation{\instSOKENDAI} % 2590
  \author{R.~Adak}\affiliation{\instFudan} % 6743
  \author{K.~Adamczyk}\affiliation{\instKrakow} % 2239
  \author{P.~Ahlburg}\affiliation{\instBonn} % 2367
  \author{J.~K.~Ahn}\affiliation{\instKorea} % 7423
  \author{H.~Aihara}\affiliation{\instUTokyo} % 2223
  \author{N.~Akopov}\affiliation{\instYerevan} % 9443
  \author{A.~Aloisio}\affiliation{\instNapoliUNIV}\affiliation{\instNapoliINFN} % 2194
  \author{F.~Ameli}\affiliation{\instRomaINFN} % 4683
  \author{L.~Andricek}\affiliation{\instMPGHLL} % 2098
  \author{N.~Anh~Ky}\affiliation{\instIOP}\affiliation{\instITAR} % 2218
  \author{D.~M.~Asner}\affiliation{\instBNL} % 4684
  \author{H.~Atmacan}\affiliation{\instCincinnati} % 2538
  \author{V.~Aulchenko}\affiliation{\instBINP}\affiliation{\instNSU} % 8183
  \author{T.~Aushev}\affiliation{\instHSE} % 3747
  \author{V.~Aushev}\affiliation{\instKyiv} % 2155
  \author{T.~Aziz}\affiliation{\instTata} % 3523
  \author{V.~Babu}\affiliation{\instDESY} % 5623
  \author{S.~Bacher}\affiliation{\instKrakow} % 2258
  \author{S.~Baehr}\affiliation{\instKarlsruhe} % 2515
  \author{S.~Bahinipati}\affiliation{\instIITBhubaneswar} % 2332
  \author{A.~M.~Bakich}\affiliation{\instSydney} % 2115
  \author{P.~Bambade}\affiliation{\instIJCLab} % 3003
  \author{Sw.~Banerjee}\affiliation{\instLouisville} % 8603
  \author{S.~Bansal}\affiliation{\instPanjab} % 5163
  \author{M.~Barrett}\affiliation{\instKEK} % 2180
  \author{G.~Batignani}\affiliation{\instPisaUNIV}\affiliation{\instPisaINFN} % 6643
  \author{J.~Baudot}\affiliation{\instIPHC} % 2562
  \author{A.~Beaulieu}\affiliation{\instVictoria} % 2444
  \author{J.~Becker}\affiliation{\instKarlsruhe} % 5403
  \author{P.~K.~Behera}\affiliation{\instIITMadras} % 4204
  \author{M.~Bender}\affiliation{\instLMU} % 2440
  \author{J.~V.~Bennett}\affiliation{\instMississippi} % 2454
  \author{E.~Bernieri}\affiliation{\instRomaTreINFN} % 4483
  \author{F.~U.~Bernlochner}\affiliation{\instBonn} % 2282
  \author{M.~Bertemes}\affiliation{\instHEPHYVienna} % 2595
  \author{M.~Bessner}\affiliation{\instHawaii} % 3783
  \author{S.~Bettarini}\affiliation{\instPisaUNIV}\affiliation{\instPisaINFN} % 2350
  \author{V.~Bhardwaj}\affiliation{\instIISER} % 2228
  \author{B.~Bhuyan}\affiliation{\instIITGuwahati} % 2097
  \author{F.~Bianchi}\affiliation{\instTorinoUNIV}\affiliation{\instTorinoINFN} % 2564
  \author{T.~Bilka}\affiliation{\instPrague} % 2484
  \author{S.~Bilokin}\affiliation{\instLMU} % 3623
  \author{D.~Biswas}\affiliation{\instLouisville} % 8703
  \author{A.~Bobrov}\affiliation{\instBINP}\affiliation{\instNSU} % 2294
  \author{A.~Bondar}\affiliation{\instBINP}\affiliation{\instNSU} % 4643
  \author{G.~Bonvicini}\affiliation{\instWayneState} % 2095
  \author{A.~Bozek}\affiliation{\instKrakow} % 2303
  \author{M.~Bra\v{c}ko}\affiliation{\instLjubljanaUM}\affiliation{\instLjubljanaJSI} % 2425
  \author{P.~Branchini}\affiliation{\instRomaTreINFN} % 2577
  \author{N.~Braun}\affiliation{\instKarlsruhe} % 2436
  \author{R.~A.~Briere}\affiliation{\instCMU} % 2584
  \author{T.~E.~Browder}\affiliation{\instHawaii} % 2560
  \author{D.~N.~Brown}\affiliation{\instLouisville} % 8743
  \author{A.~Budano}\affiliation{\instRomaTreINFN} % 2171
  \author{L.~Burmistrov}\affiliation{\instIJCLab} % 2111
  \author{S.~Bussino}\affiliation{\instRomaTreUNIV}\affiliation{\instRomaTreINFN} % 5384
  \author{M.~Campajola}\affiliation{\instNapoliUNIV}\affiliation{\instNapoliINFN} % 5223
  \author{L.~Cao}\affiliation{\instBonn} % 2099
  \author{G.~Caria}\affiliation{\instMelbourne} % 2438
  \author{G.~Casarosa}\affiliation{\instPisaUNIV}\affiliation{\instPisaINFN} % 2491
  \author{C.~Cecchi}\affiliation{\instPerugiaUNIV}\affiliation{\instPerugiaINFN} % 2433
  \author{D.~\v{C}ervenkov}\affiliation{\instPrague} % 2078
  \author{M.-C.~Chang}\affiliation{\instFuJen} % 2827
  \author{P.~Chang}\affiliation{\instNTUTaiwan} % 2542
  \author{R.~Cheaib}\affiliation{\instUBC} % 2208
  \author{V.~Chekelian}\affiliation{\instMPP} % 2167
  \author{Y.~Q.~Chen}\affiliation{\instUSTC} % 2576
  \author{Y.-T.~Chen}\affiliation{\instNTUTaiwan} % 2884
  \author{B.~G.~Cheon}\affiliation{\instHanyang} % 2173
  \author{K.~Chilikin}\affiliation{\instLPI} % 2308
  \author{K.~Chirapatpimol}\affiliation{\instChiangMai} % 10803
  \author{H.-E.~Cho}\affiliation{\instHanyang} % 2182
  \author{K.~Cho}\affiliation{\instKISTI} % 2516
  \author{S.-J.~Cho}\affiliation{\instYonsei} % 2723
  \author{S.-K.~Choi}\affiliation{\instGyeongsang} % 2364
  \author{S.~Choudhury}\affiliation{\instIITHyderabad} % 2206
  \author{D.~Cinabro}\affiliation{\instWayneState} % 2092
  \author{L.~Corona}\affiliation{\instPisaUNIV}\affiliation{\instPisaINFN} % 3944
  \author{L.~M.~Cremaldi}\affiliation{\instMississippi} % 2276
  \author{D.~Cuesta}\affiliation{\instIPHC} % 2668
  \author{S.~Cunliffe}\affiliation{\instDESY} % 2272
  \author{T.~Czank}\affiliation{\instIPMU} % 2254
  \author{N.~Dash}\affiliation{\instIITMadras} % 2601
  \author{F.~Dattola}\affiliation{\instDESY} % 3745
  \author{E.~De~La~Cruz-Burelo}\affiliation{\instCinvestavIPN} % 2359
  \author{G.~De~Nardo}\affiliation{\instNapoliUNIV}\affiliation{\instNapoliINFN} % 2459
  \author{M.~De~Nuccio}\affiliation{\instDESY} % 2610
  \author{G.~De~Pietro}\affiliation{\instRomaTreINFN} % 2528
  \author{R.~de~Sangro}\affiliation{\instFrascati} % 2524
  \author{B.~Deschamps}\affiliation{\instBonn} % 2671
  \author{M.~Destefanis}\affiliation{\instTorinoUNIV}\affiliation{\instTorinoINFN} % 2594
  \author{S.~Dey}\affiliation{\instTelAviv} % 5023
  \author{A.~De~Yta-Hernandez}\affiliation{\instCinvestavIPN} % 2104
  \author{A.~Di~Canto}\affiliation{\instBNL} % 10963
  \author{F.~Di~Capua}\affiliation{\instNapoliUNIV}\affiliation{\instNapoliINFN} % 2065
  \author{S.~Di~Carlo}\affiliation{\instIJCLab} % 2079
  \author{J.~Dingfelder}\affiliation{\instBonn} % 2151
  \author{Z.~Dole\v{z}al}\affiliation{\instPrague} % 2319
  \author{I.~Dom\'{\i}nguez~Jim\'{e}nez}\affiliation{\instUAS} % 2191
  \author{T.~V.~Dong}\affiliation{\instFudan} % 2215
  \author{K.~Dort}\affiliation{\instGiessen} % 5583
  \author{D.~Dossett}\affiliation{\instMelbourne} % 2574
  \author{S.~Dubey}\affiliation{\instHawaii} % 11063
  \author{S.~Duell}\affiliation{\instBonn} % 2344
  \author{G.~Dujany}\affiliation{\instIPHC} % 9703
  \author{S.~Eidelman}\affiliation{\instBINP}\affiliation{\instLPI}\affiliation{\instNSU} % 4984
  \author{M.~Eliachevitch}\affiliation{\instBonn} % 2725
  \author{D.~Epifanov}\affiliation{\instBINP}\affiliation{\instNSU} % 2551
  \author{J.~E.~Fast}\affiliation{\instPNNL} % 2264
  \author{T.~Ferber}\affiliation{\instDESY} % 2482
  \author{D.~Ferlewicz}\affiliation{\instMelbourne} % 2073
  \author{G.~Finocchiaro}\affiliation{\instFrascati} % 2400
  \author{S.~Fiore}\affiliation{\instRomaINFN} % 4225
  \author{P.~Fischer}\affiliation{\instHeidelberg} % 2141
  \author{A.~Fodor}\affiliation{\instMcGill} % 2312
  \author{F.~Forti}\affiliation{\instPisaUNIV}\affiliation{\instPisaINFN} % 2432
  \author{A.~Frey}\affiliation{\instGoettingen} % 2150
  \author{M.~Friedl}\affiliation{\instHEPHYVienna} % 2442
  \author{B.~G.~Fulsom}\affiliation{\instPNNL} % 2563
  \author{M.~Gabriel}\affiliation{\instMPP} % 2443
  \author{N.~Gabyshev}\affiliation{\instBINP}\affiliation{\instNSU} % 2510
  \author{E.~Ganiev}\affiliation{\instTriesteUNIV}\affiliation{\instTriesteINFN} % 4623
  \author{M.~Garcia-Hernandez}\affiliation{\instCinvestavIPN} % 4823
  \author{R.~Garg}\affiliation{\instPanjab} % 2213
  \author{A.~Garmash}\affiliation{\instBINP}\affiliation{\instNSU} % 2161
  \author{V.~Gaur}\affiliation{\instVPI} % 2413
  \author{A.~Gaz}\affiliation{\instNagoya}\affiliation{\instNagoyaKMI} % 2181
  \author{U.~Gebauer}\affiliation{\instGoettingen} % 2174
  \author{M.~Gelb}\affiliation{\instKarlsruhe} % 2340
  \author{A.~Gellrich}\affiliation{\instDESY} % 2480
  \author{J.~Gemmler}\affiliation{\instKarlsruhe} % 2321
  \author{T.~Ge{\ss}ler}\affiliation{\instGiessen} % 2121
  \author{D.~Getzkow}\affiliation{\instGiessen} % 2416
  \author{R.~Giordano}\affiliation{\instNapoliUNIV}\affiliation{\instNapoliINFN} % 2103
  \author{A.~Giri}\affiliation{\instIITHyderabad} % 2106
  \author{A.~Glazov}\affiliation{\instDESY} % 2473
  \author{B.~Gobbo}\affiliation{\instTriesteINFN} % 2109
  \author{R.~Godang}\affiliation{\instSAlabama} % 2449
  \author{P.~Goldenzweig}\affiliation{\instKarlsruhe} % 2345
  \author{B.~Golob}\affiliation{\instLjubljanaUniLJ}\affiliation{\instLjubljanaJSI} % 3703
  \author{P.~Gomis}\affiliation{\instIFIC} % 2354
  \author{P.~Grace}\affiliation{\instAdelaide} % 9563
  \author{W.~Gradl}\affiliation{\instMainz} % 2570
  \author{E.~Graziani}\affiliation{\instRomaTreINFN} % 2342
  \author{D.~Greenwald}\affiliation{\instTUM} % 2686
  \author{Y.~Guan}\affiliation{\instCincinnati} % 2514
  \author{C.~Hadjivasiliou}\affiliation{\instPNNL} % 9503
  \author{S.~Halder}\affiliation{\instTata} % 4743
  \author{K.~Hara}\affiliation{\instKEK}\affiliation{\instSOKENDAI} % 2462
  \author{T.~Hara}\affiliation{\instKEK}\affiliation{\instSOKENDAI} % 2523
  \author{O.~Hartbrich}\affiliation{\instHawaii} % 2158
  \author{T.~Hauth}\affiliation{\instKarlsruhe} % 2553
  \author{K.~Hayasaka}\affiliation{\instNiigata} % 2330
  \author{H.~Hayashii}\affiliation{\instNaraWu} % 2455
  \author{C.~Hearty}\affiliation{\instUBC}\affiliation{\instIPP} % 2450
  \author{M.~Heck}\affiliation{\instKarlsruhe} % 2561
  \author{M.~T.~Hedges}\affiliation{\instHawaii} % 2265
  \author{I.~Heredia~de~la~Cruz}\affiliation{\instCinvestavIPN}\affiliation{\instConacyt} % 2559
  \author{M.~Hern\'{a}ndez~Villanueva}\affiliation{\instMississippi} % 2466
  \author{A.~Hershenhorn}\affiliation{\instUBC} % 2552
  \author{T.~Higuchi}\affiliation{\instIPMU} % 2485
  \author{E.~C.~Hill}\affiliation{\instUBC} % 7823
  \author{H.~Hirata}\affiliation{\instNagoya} % 2070
  \author{M.~Hoek}\affiliation{\instMainz} % 2101
  \author{M.~Hohmann}\affiliation{\instMelbourne} % 2077
  \author{S.~Hollitt}\affiliation{\instAdelaide} % 2557
  \author{T.~Hotta}\affiliation{\instRCNP} % 2084
  \author{C.-L.~Hsu}\affiliation{\instSydney} % 2299
  \author{Y.~Hu}\affiliation{\instIHEPChina} % 2227
  \author{K.~Huang}\affiliation{\instNTUTaiwan} % 2389
  \author{T.~Iijima}\affiliation{\instNagoya}\affiliation{\instNagoyaKMI} % 2446
  \author{K.~Inami}\affiliation{\instNagoya} % 2323
  \author{G.~Inguglia}\affiliation{\instHEPHYVienna} % 2500
  \author{J.~Irakkathil~Jabbar}\affiliation{\instKarlsruhe} % 7343
  \author{A.~Ishikawa}\affiliation{\instKEK}\affiliation{\instSOKENDAI} % 2281
  \author{R.~Itoh}\affiliation{\instKEK}\affiliation{\instSOKENDAI} % 2487
  \author{M.~Iwasaki}\affiliation{\instOsakaCity} % 2360
  \author{Y.~Iwasaki}\affiliation{\instKEK} % 2229
  \author{S.~Iwata}\affiliation{\instTokyoMetropolitan} % 4323
  \author{P.~Jackson}\affiliation{\instAdelaide} % 2255
  \author{W.~W.~Jacobs}\affiliation{\instIndiana} % 2322
  \author{I.~Jaegle}\affiliation{\instFlorida} % 2539
  \author{D.~E.~Jaffe}\affiliation{\instBNL} % 3663
  \author{E.-J.~Jang}\affiliation{\instGyeongsang} % 6744
  \author{M.~Jeandron}\affiliation{\instMississippi} % 2806
  \author{H.~B.~Jeon}\affiliation{\instKyungpook} % 2170
  \author{S.~Jia}\affiliation{\instFudan} % 2457
  \author{Y.~Jin}\affiliation{\instTriesteINFN} % 2105
  \author{C.~Joo}\affiliation{\instIPMU} % 3525
  \author{K.~K.~Joo}\affiliation{\instChonnam} % 4224
  \author{I.~Kadenko}\affiliation{\instKyiv} % 3843
  \author{J.~Kahn}\affiliation{\instKarlsruhe} % 2448
  \author{H.~Kakuno}\affiliation{\instTokyoMetropolitan} % 2391
  \author{A.~B.~Kaliyar}\affiliation{\instTata} % 7344
  \author{J.~Kandra}\affiliation{\instPrague} % 2541
  \author{K.~H.~Kang}\affiliation{\instKyungpook} % 2283
  \author{P.~Kapusta}\affiliation{\instKrakow} % 6663
  \author{R.~Karl}\affiliation{\instDESY} % 10923
  \author{G.~Karyan}\affiliation{\instYerevan} % 2550
  \author{Y.~Kato}\affiliation{\instNagoya}\affiliation{\instNagoyaKMI} % 2549
  \author{H.~Kawai}\affiliation{\instChiba} % 4344
  \author{T.~Kawasaki}\affiliation{\instKitasato} % 4363
  \author{T.~Keck}\affiliation{\instKarlsruhe} % 2300
  \author{C.~Ketter}\affiliation{\instHawaii} % 2236
  \author{H.~Kichimi}\affiliation{\instKEK} % 2233
  \author{C.~Kiesling}\affiliation{\instMPP} % 2168
  \author{B.~H.~Kim}\affiliation{\instSeoul} % 9743
  \author{C.-H.~Kim}\affiliation{\instHanyang} % 2358
  \author{D.~Y.~Kim}\affiliation{\instSoongsil} % 2315
  \author{H.~J.~Kim}\affiliation{\instKyungpook} % 4863
  \author{J.~B.~Kim}\affiliation{\instKorea} % 2408
  \author{K.-H.~Kim}\affiliation{\instYonsei} % 2118
  \author{K.~Kim}\affiliation{\instKorea} % 2409
  \author{S.-H.~Kim}\affiliation{\instSeoul} % 2428
  \author{Y.-K.~Kim}\affiliation{\instYonsei} % 2379
  \author{Y.~Kim}\affiliation{\instKorea} % 2403
  \author{T.~D.~Kimmel}\affiliation{\instVPI} % 2241
  \author{H.~Kindo}\affiliation{\instKEK}\affiliation{\instSOKENDAI} % 2195
  \author{K.~Kinoshita}\affiliation{\instCincinnati} % 2318
  \author{B.~Kirby}\affiliation{\instBNL} % 5263
  \author{C.~Kleinwort}\affiliation{\instDESY} % 2499
  \author{B.~Knysh}\affiliation{\instIJCLab} % 8883
  \author{P.~Kody\v{s}}\affiliation{\instPrague} % 2407
  \author{T.~Koga}\affiliation{\instKEK} % 6963
  \author{S.~Kohani}\affiliation{\instHawaii} % 9143
  \author{I.~Komarov}\affiliation{\instDESY} % 2210
  \author{T.~Konno}\affiliation{\instKitasato} % 2490
  \author{S.~Korpar}\affiliation{\instLjubljanaUM}\affiliation{\instLjubljanaJSI} % 2475
% \author{E.~Kou}\affiliation{\instIJCLab} % 3765
  \author{N.~Kovalchuk}\affiliation{\instDESY} % 6964
  \author{T.~M.~G.~Kraetzschmar}\affiliation{\instMPP} % 7543
  \author{P.~Kri\v{z}an}\affiliation{\instLjubljanaUniLJ}\affiliation{\instLjubljanaJSI} % 2474
  \author{R.~Kroeger}\affiliation{\instMississippi} % 2242
  \author{J.~F.~Krohn}\affiliation{\instMelbourne} % 2502
  \author{P.~Krokovny}\affiliation{\instBINP}\affiliation{\instNSU} % 2575
  \author{H.~Kr\"uger}\affiliation{\instBonn} % 2290
  \author{W.~Kuehn}\affiliation{\instGiessen} % 2534
  \author{T.~Kuhr}\affiliation{\instLMU} % 2486
  \author{J.~Kumar}\affiliation{\instCMU} % 6464
  \author{M.~Kumar}\affiliation{\instMNITJaipur} % 2744
  \author{R.~Kumar}\affiliation{\instPanjabPAU} % 2189
  \author{K.~Kumara}\affiliation{\instWayneState} % 2257
  \author{T.~Kumita}\affiliation{\instTokyoMetropolitan} % 4083
  \author{T.~Kunigo}\affiliation{\instKEK} % 10104
  \author{M.~K\"{u}nzel}\affiliation{\instDESY}\affiliation{\instLMU} % 2139
  \author{S.~Kurz}\affiliation{\instDESY} % 9363
  \author{A.~Kuzmin}\affiliation{\instBINP}\affiliation{\instNSU} % 2520
  \author{P.~Kvasni\v{c}ka}\affiliation{\instPrague} % 2184
  \author{Y.-J.~Kwon}\affiliation{\instYonsei} % 2231
  \author{S.~Lacaprara}\affiliation{\instPadovaINFN} % 2447
  \author{Y.-T.~Lai}\affiliation{\instIPMU} % 2066
  \author{C.~La~Licata}\affiliation{\instIPMU} % 2348
  \author{K.~Lalwani}\affiliation{\instMNITJaipur} % 2142
  \author{L.~Lanceri}\affiliation{\instTriesteINFN} % 2540
  \author{J.~S.~Lange}\affiliation{\instGiessen} % 2277
  \author{K.~Lautenbach}\affiliation{\instGiessen} % 2102
  \author{P.~J.~Laycock}\affiliation{\instBNL} % 7683
  \author{F.~R.~Le~Diberder}\affiliation{\instIJCLab} % 3267
  \author{I.-S.~Lee}\affiliation{\instHanyang} % 2422
  \author{S.~C.~Lee}\affiliation{\instKyungpook} % 2544
  \author{P.~Leitl}\affiliation{\instMPP} % 2414
  \author{D.~Levit}\affiliation{\instTUM} % 2507
  \author{P.~M.~Lewis}\affiliation{\instBonn} % 2582
  \author{C.~Li}\affiliation{\instLNNU} % 2325
  \author{L.~K.~Li}\affiliation{\instCincinnati} % 3263
  \author{S.~X.~Li}\affiliation{\instBeihang} % 2377
  \author{Y.~M.~Li}\affiliation{\instIHEPChina} % 2203
  \author{Y.~B.~Li}\affiliation{\instPeking} % 2573
  \author{J.~Libby}\affiliation{\instIITMadras} % 2262
  \author{K.~Lieret}\affiliation{\instLMU} % 2268
  \author{L.~Li~Gioi}\affiliation{\instMPP} % 2495
  \author{J.~Lin}\affiliation{\instNTUTaiwan} % 2401
  \author{Z.~Liptak}\affiliation{\instHawaii} % 3565
  \author{Q.~Y.~Liu}\affiliation{\instDESY} % 7045
  \author{Z.~A.~Liu}\affiliation{\instIHEPChina} % 3283
  \author{D.~Liventsev}\affiliation{\instWayneState}\affiliation{\instKEK} % 2578
  \author{S.~Longo}\affiliation{\instDESY} % 2396
  \author{A.~Loos}\affiliation{\instSCarolina} % 2356
  \author{P.~Lu}\affiliation{\instNTUTaiwan} % 2148
  \author{M.~Lubej}\affiliation{\instLjubljanaJSI} % 2513
  \author{T.~Lueck}\affiliation{\instLMU} % 2406
  \author{F.~Luetticke}\affiliation{\instBonn} % 2533
  \author{T.~Luo}\affiliation{\instFudan} % 3268
  \author{C.~MacQueen}\affiliation{\instMelbourne} % 2585
  \author{Y.~Maeda}\affiliation{\instNagoya}\affiliation{\instNagoyaKMI} % 2427
  \author{M.~Maggiora}\affiliation{\instTorinoUNIV}\affiliation{\instTorinoINFN} % 5343
  \author{S.~Maity}\affiliation{\instIITBhubaneswar} % 2985
  \author{R.~Manfredi}\affiliation{\instTriesteUNIV}\affiliation{\instTriesteINFN} % 10303
  \author{E.~Manoni}\affiliation{\instPerugiaINFN} % 2305
  \author{S.~Marcello}\affiliation{\instTorinoUNIV}\affiliation{\instTorinoINFN} % 4223
  \author{C.~Marinas}\affiliation{\instIFIC} % 2133
  \author{A.~Martini}\affiliation{\instRomaTreUNIV}\affiliation{\instRomaTreINFN} % 2336
  \author{M.~Masuda}\affiliation{\instEri}\affiliation{\instRCNP} % 2238
  \author{T.~Matsuda}\affiliation{\instUOM} % 5543
  \author{K.~Matsuoka}\affiliation{\instNagoya}\affiliation{\instNagoyaKMI} % 2316
  \author{D.~Matvienko}\affiliation{\instBINP}\affiliation{\instLPI}\affiliation{\instNSU} % 2351
  \author{J.~McNeil}\affiliation{\instFlorida} % 2382
  \author{F.~Meggendorfer}\affiliation{\instMPP} % 7103
  \author{J.~C.~Mei}\affiliation{\instFudan} % 7404
  \author{F.~Meier}\affiliation{\instDuke} % 3103
  \author{M.~Merola}\affiliation{\instNapoliUNIV}\affiliation{\instNapoliINFN} % 2456
  \author{F.~Metzner}\affiliation{\instKarlsruhe} % 2296
  \author{M.~Milesi}\affiliation{\instMelbourne} % 5443
  \author{C.~Miller}\affiliation{\instVictoria} % 2273
  \author{K.~Miyabayashi}\affiliation{\instNaraWu} % 2327
  \author{H.~Miyake}\affiliation{\instKEK}\affiliation{\instSOKENDAI} % 2452
  \author{H.~Miyata}\affiliation{\instNiigata} % 2071
  \author{R.~Mizuk}\affiliation{\instLPI}\affiliation{\instHSE} % 2483
  \author{K.~Azmi}\affiliation{\instMalaya} % 2506
  \author{G.~B.~Mohanty}\affiliation{\instTata} % 2278
  \author{H.~Moon}\affiliation{\instKorea} % 2304
  \author{T.~Moon}\affiliation{\instSeoul} % 2397
  \author{J.~A.~Mora~Grimaldo}\affiliation{\instUTokyo} % 4403
  \author{A.~Morda}\affiliation{\instPadovaINFN} % 2503
  \author{T.~Morii}\affiliation{\instIPMU} % 3543
  \author{H.-G.~Moser}\affiliation{\instMPP} % 2120
  \author{M.~Mrvar}\affiliation{\instHEPHYVienna} % 2527
  \author{F.~Mueller}\affiliation{\instMPP} % 2240
  \author{F.~J.~M\"{u}ller}\affiliation{\instDESY} % 2123
  \author{Th.~Muller}\affiliation{\instKarlsruhe} % 2165
  \author{G.~Muroyama}\affiliation{\instNagoya} % 2093
  \author{C.~Murphy}\affiliation{\instIPMU} % 12403
  \author{R.~Mussa}\affiliation{\instTorinoINFN} % 2372
  \author{K.~Nakagiri}\affiliation{\instKEK} % 10103
  \author{I.~Nakamura}\affiliation{\instKEK}\affiliation{\instSOKENDAI} % 3463
  \author{K.~R.~Nakamura}\affiliation{\instKEK}\affiliation{\instSOKENDAI} % 2417
  \author{E.~Nakano}\affiliation{\instOsakaCity} % 2554
  \author{M.~Nakao}\affiliation{\instKEK}\affiliation{\instSOKENDAI} % 2498
  \author{H.~Nakayama}\affiliation{\instKEK}\affiliation{\instSOKENDAI} % 2232
  \author{H.~Nakazawa}\affiliation{\instNTUTaiwan} % 2335
  \author{T.~Nanut}\affiliation{\instLjubljanaJSI} % 2565
  \author{Z.~Natkaniec}\affiliation{\instKrakow} % 3923
  \author{A.~Natochii}\affiliation{\instHawaii} % 12063
  \author{M.~Nayak}\affiliation{\instTelAviv} % 2371
  \author{G.~Nazaryan}\affiliation{\instYerevan} % 9523
  \author{D.~Neverov}\affiliation{\instNagoya} % 2075
  \author{C.~Niebuhr}\affiliation{\instDESY} % 2477
  \author{M.~Niiyama}\affiliation{\instKSU} % 2063
  \author{J.~Ninkovic}\affiliation{\instMPGHLL} % 2386
  \author{N.~K.~Nisar}\affiliation{\instBNL} % 2522
  \author{S.~Nishida}\affiliation{\instKEK}\affiliation{\instSOKENDAI} % 2571
  \author{K.~Nishimura}\affiliation{\instHawaii} % 3063
  \author{M.~Nishimura}\affiliation{\instKEK} % 7743
  \author{M.~H.~A.~Nouxman}\affiliation{\instMalaya} % 2470
  \author{B.~Oberhof}\affiliation{\instFrascati} % 2393
  \author{K.~Ogawa}\affiliation{\instNiigata} % 2430
  \author{S.~Ogawa}\affiliation{\instToho} % 6263
  \author{S.~L.~Olsen}\affiliation{\instGyeongsang} % 4563
  \author{Y.~Onishchuk}\affiliation{\instKyiv} % 2157
  \author{H.~Ono}\affiliation{\instNiigata} % 2160
  \author{Y.~Onuki}\affiliation{\instUTokyo} % 2331
  \author{P.~Oskin}\affiliation{\instLPI} % 9623
  \author{E.~R.~Oxford}\affiliation{\instCMU} % 6943
  \author{H.~Ozaki}\affiliation{\instKEK}\affiliation{\instSOKENDAI} % 2984
  \author{P.~Pakhlov}\affiliation{\instLPI}\affiliation{\instMEPhI} % 2221
  \author{G.~Pakhlova}\affiliation{\instHSE}\affiliation{\instLPI} % 2188
  \author{A.~Paladino}\affiliation{\instPisaUNIV}\affiliation{\instPisaINFN} % 2435
  \author{T.~Pang}\affiliation{\instPittsburgh} % 2114
  \author{A.~Panta}\affiliation{\instMississippi} % 7943
  \author{E.~Paoloni}\affiliation{\instPisaUNIV}\affiliation{\instPisaINFN} % 2488
  \author{S.~Pardi}\affiliation{\instNapoliINFN} % 2532
  \author{C.~Park}\affiliation{\instYonsei} % 2307
  \author{H.~Park}\affiliation{\instKyungpook} % 2284
  \author{S.-H.~Park}\affiliation{\instYonsei} % 2509
  \author{B.~Paschen}\affiliation{\instBonn} % 2159
  \author{A.~Passeri}\affiliation{\instRomaTreINFN} % 2116
  \author{A.~Pathak}\affiliation{\instLouisville} % 8723
  \author{S.~Patra}\affiliation{\instIISER} % 3123
  \author{S.~Paul}\affiliation{\instTUM} % 2131
  \author{T.~K.~Pedlar}\affiliation{\instLuther} % 2421
  \author{I.~Peruzzi}\affiliation{\instFrascati} % 2253
  \author{R.~Peschke}\affiliation{\instHawaii} % 7123
  \author{R.~Pestotnik}\affiliation{\instLjubljanaJSI} % 2476
  \author{M.~Piccolo}\affiliation{\instFrascati} % 2147
  \author{L.~E.~Piilonen}\affiliation{\instVPI} % 2346
  \author{P.~L.~M.~Podesta-Lerma}\affiliation{\instUAS} % 2266
  \author{G.~Polat}\affiliation{\instCPPM} % 9783
  \author{V.~Popov}\affiliation{\instHSE} % 2096
  \author{C.~Praz}\affiliation{\instDESY} % 2726
  \author{E.~Prencipe}\affiliation{\instJuelich} % 2219
  \author{M.~T.~Prim}\affiliation{\instBonn} % 2501
  \author{M.~V.~Purohit}\affiliation{\instOkinawa} % 2196
  \author{N.~Rad}\affiliation{\instDESY} % 11683
  \author{P.~Rados}\affiliation{\instDESY} % 7383
  \author{R.~Rasheed}\affiliation{\instIPHC} % 3643
  \author{M.~Reif}\affiliation{\instMPP} % 8043
  \author{S.~Reiter}\affiliation{\instGiessen} % 2248
  \author{M.~Remnev}\affiliation{\instBINP}\affiliation{\instNSU} % 2785
  \author{P.~K.~Resmi}\affiliation{\instIITMadras} % 2588
  \author{I.~Ripp-Baudot}\affiliation{\instIPHC} % 2469
  \author{M.~Ritter}\affiliation{\instLMU} % 2580
  \author{M.~Ritzert}\affiliation{\instHeidelberg} % 2526
  \author{G.~Rizzo}\affiliation{\instPisaUNIV}\affiliation{\instPisaINFN} % 2579
  \author{L.~B.~Rizzuto}\affiliation{\instLjubljanaJSI} % 3746
  \author{S.~H.~Robertson}\affiliation{\instMcGill}\affiliation{\instIPP} % 2471
  \author{D.~Rodr\'{i}guez~P\'{e}rez}\affiliation{\instUAS} % 2176
  \author{J.~M.~Roney}\affiliation{\instVictoria}\affiliation{\instIPP} % 2244
  \author{C.~Rosenfeld}\affiliation{\instSCarolina} % 2082
  \author{A.~Rostomyan}\affiliation{\instDESY} % 2481
  \author{N.~Rout}\affiliation{\instIITMadras} % 2965
  \author{M.~Rozanska}\affiliation{\instKrakow} % 2205
  \author{G.~Russo}\affiliation{\instNapoliUNIV}\affiliation{\instNapoliINFN} % 2388
  \author{D.~Sahoo}\affiliation{\instTata} % 2110
  \author{Y.~Sakai}\affiliation{\instKEK}\affiliation{\instSOKENDAI} % 2175
  \author{D.~A.~Sanders}\affiliation{\instMississippi} % 2458
  \author{S.~Sandilya}\affiliation{\instCincinnati} % 2286
  \author{A.~Sangal}\affiliation{\instCincinnati} % 2384
  \author{L.~Santelj}\affiliation{\instLjubljanaUniLJ}\affiliation{\instLjubljanaJSI} % 2185
  \author{P.~Sartori}\affiliation{\instPadovaUNIV}\affiliation{\instPadovaINFN} % 4523
  \author{J.~Sasaki}\affiliation{\instUTokyo} % 4383
  \author{Y.~Sato}\affiliation{\instTohoku} % 5243
  \author{V.~Savinov}\affiliation{\instPittsburgh} % 2292
  \author{B.~Scavino}\affiliation{\instMainz} % 2518
  \author{M.~Schram}\affiliation{\instPNNL} % 2306
  \author{H.~Schreeck}\affiliation{\instGoettingen} % 2434
  \author{J.~Schueler}\affiliation{\instHawaii} % 2824
  \author{C.~Schwanda}\affiliation{\instHEPHYVienna} % 2108
  \author{A.~J.~Schwartz}\affiliation{\instCincinnati} % 2162
  \author{B.~Schwenker}\affiliation{\instGoettingen} % 2405
  \author{R.~M.~Seddon}\affiliation{\instMcGill} % 2314
  \author{Y.~Seino}\affiliation{\instNiigata} % 2517
  \author{A.~Selce}\affiliation{\instRomaUNIV}\affiliation{\instRomaINFN} % 9043
  \author{K.~Senyo}\affiliation{\instYamagata} % 2987
  \author{I.~S.~Seong}\affiliation{\instHawaii} % 2572
  \author{J.~Serrano}\affiliation{\instCPPM} % 12124
  \author{M.~E.~Sevior}\affiliation{\instMelbourne} % 2328
  \author{C.~Sfienti}\affiliation{\instMainz} % 2214
  \author{V.~Shebalin}\affiliation{\instHawaii} % 2339
  \author{C.~P.~Shen}\affiliation{\instBeihang} % 2464
  \author{H.~Shibuya}\affiliation{\instToho} % 2234
  \author{J.-G.~Shiu}\affiliation{\instNTUTaiwan} % 2412
  \author{B.~Shwartz}\affiliation{\instBINP}\affiliation{\instNSU} % 2122
  \author{A.~Sibidanov}\affiliation{\instVictoria} % 2419
  \author{F.~Simon}\affiliation{\instMPP} % 2164
  \author{J.~B.~Singh}\affiliation{\instPanjab} % 2903
  \author{S.~Skambraks}\affiliation{\instMPP} % 2394
  \author{K.~Smith}\affiliation{\instMelbourne} % 2243
  \author{R.~J.~Sobie}\affiliation{\instVictoria}\affiliation{\instIPP} % 2472
  \author{A.~Soffer}\affiliation{\instTelAviv} % 2217
  \author{A.~Sokolov}\affiliation{\instIHEPRussia} % 2521
  \author{Y.~Soloviev}\affiliation{\instDESY} % 2479
  \author{E.~Solovieva}\affiliation{\instLPI} % 2398
  \author{S.~Spataro}\affiliation{\instTorinoUNIV}\affiliation{\instTorinoINFN} % 2117
  \author{B.~Spruck}\affiliation{\instMainz} % 2493
  \author{M.~Stari\v{c}}\affiliation{\instLjubljanaJSI} % 2326
  \author{S.~Stefkova}\affiliation{\instDESY} % 8783
  \author{Z.~S.~Stottler}\affiliation{\instVPI} % 2267
  \author{R.~Stroili}\affiliation{\instPadovaUNIV}\affiliation{\instPadovaINFN} % 2465
  \author{J.~Strube}\affiliation{\instPNNL} % 2451
  \author{J.~Stypula}\affiliation{\instKrakow} % 2368
  \author{M.~Sumihama}\affiliation{\instGifu}\affiliation{\instRCNP} % 4243
  \author{K.~Sumisawa}\affiliation{\instKEK}\affiliation{\instSOKENDAI} % 2583
  \author{T.~Sumiyoshi}\affiliation{\instTokyoMetropolitan} % 4184
  \author{D.~J.~Summers}\affiliation{\instMississippi} % 7405
  \author{W.~Sutcliffe}\affiliation{\instBonn} % 3784
  \author{K.~Suzuki}\affiliation{\instNagoya} % 2445
  \author{S.~Y.~Suzuki}\affiliation{\instKEK}\affiliation{\instSOKENDAI} % 2496
  \author{H.~Svidras}\affiliation{\instDESY} % 11783
  \author{M.~Tabata}\affiliation{\instChiba} % 2986
  \author{M.~Takahashi}\affiliation{\instDESY} % 2467
  \author{M.~Takizawa}\affiliation{\instRIKENMSL}\affiliation{\instJPARC}\affiliation{\instSPU} % 2437
  \author{U.~Tamponi}\affiliation{\instTorinoINFN} % 2366
  \author{S.~Tanaka}\affiliation{\instKEK}\affiliation{\instSOKENDAI} % 2530
  \author{K.~Tanida}\affiliation{\instJAEA} % 3803
  \author{H.~Tanigawa}\affiliation{\instUTokyo} % 2237
  \author{N.~Taniguchi}\affiliation{\instKEK} % 2285
  \author{Y.~Tao}\affiliation{\instFlorida} % 2362
  \author{P.~Taras}\affiliation{\instMontreal} % 2202
  \author{F.~Tenchini}\affiliation{\instDESY} % 2546
  \author{D.~Tonelli}\affiliation{\instTriesteINFN} % 4564
  \author{E.~Torassa}\affiliation{\instPadovaINFN} % 2556
  \author{K.~Trabelsi}\affiliation{\instIJCLab} % 2369
  \author{T.~Tsuboyama}\affiliation{\instKEK}\affiliation{\instSOKENDAI} % 2361
  \author{N.~Tsuzuki}\affiliation{\instNagoya} % 2352
  \author{M.~Uchida}\affiliation{\instTitech} % 2370
  \author{I.~Ueda}\affiliation{\instKEK}\affiliation{\instSOKENDAI} % 2519
  \author{S.~Uehara}\affiliation{\instKEK}\affiliation{\instSOKENDAI} % 2586
  \author{T.~Ueno}\affiliation{\instTohoku} % 4364
  \author{T.~Uglov}\affiliation{\instLPI}\affiliation{\instHSE} % 2252
  \author{K.~Unger}\affiliation{\instKarlsruhe} % 9463
  \author{Y.~Unno}\affiliation{\instHanyang} % 2420
  \author{S.~Uno}\affiliation{\instKEK}\affiliation{\instSOKENDAI} % 2149
  \author{P.~Urquijo}\affiliation{\instMelbourne} % 2302
  \author{Y.~Ushiroda}\affiliation{\instKEK}\affiliation{\instSOKENDAI}\affiliation{\instUTokyo} % 2317
  \author{Y.~Usov}\affiliation{\instBINP}\affiliation{\instNSU} % 5003
  \author{S.~E.~Vahsen}\affiliation{\instHawaii} % 2251
  \author{R.~van~Tonder}\affiliation{\instBonn} % 2706
  \author{G.~S.~Varner}\affiliation{\instHawaii} % 2119
  \author{K.~E.~Varvell}\affiliation{\instSydney} % 2545
  \author{A.~Vinokurova}\affiliation{\instBINP}\affiliation{\instNSU} % 2289
  \author{L.~Vitale}\affiliation{\instTriesteUNIV}\affiliation{\instTriesteINFN} % 2415
  \author{V.~Vorobyev}\affiliation{\instBINP}\affiliation{\instLPI}\affiliation{\instNSU} % 2298
  \author{A.~Vossen}\affiliation{\instDuke} % 2249
  \author{E.~Waheed}\affiliation{\instKEK} % 2226
  \author{H.~M.~Wakeling}\affiliation{\instMcGill} % 3664
  \author{K.~Wan}\affiliation{\instUTokyo} % 2591
  \author{W.~Wan~Abdullah}\affiliation{\instMalaya} % 2280
  \author{B.~Wang}\affiliation{\instMPP} % 2569
  \author{C.~H.~Wang}\affiliation{\instNUUTaiwan} % 2224
  \author{M.-Z.~Wang}\affiliation{\instNTUTaiwan} % 2074
  \author{X.~L.~Wang}\affiliation{\instFudan} % 2076
  \author{A.~Warburton}\affiliation{\instMcGill} % 2347
  \author{M.~Watanabe}\affiliation{\instNiigata} % 2309
  \author{S.~Watanuki}\affiliation{\instIJCLab} % 6843
  \author{I.~Watson}\affiliation{\instUTokyo} % 2337
  \author{J.~Webb}\affiliation{\instMelbourne} % 2423
  \author{S.~Wehle}\affiliation{\instDESY} % 2489
  \author{M.~Welsch}\affiliation{\instBonn} % 7023
  \author{C.~Wessel}\affiliation{\instBonn} % 2100
  \author{J.~Wiechczynski}\affiliation{\instPisaINFN} % 2604
  \author{P.~Wieduwilt}\affiliation{\instGoettingen} % 2343
  \author{H.~Windel}\affiliation{\instMPP} % 2081
  \author{E.~Won}\affiliation{\instKorea} % 2410
  \author{L.~J.~Wu}\affiliation{\instIHEPChina} % 2704
  \author{X.~P.~Xu}\affiliation{\instSoochow} % 4923
  \author{B.~Yabsley}\affiliation{\instSydney} % 3645
  \author{S.~Yamada}\affiliation{\instKEK} % 2492
  \author{W.~Yan}\affiliation{\instUSTC} % 2094
  \author{S.~B.~Yang}\affiliation{\instKorea} % 2374
  \author{H.~Ye}\affiliation{\instDESY} % 2537
  \author{J.~Yelton}\affiliation{\instFlorida} % 2067
  \author{I.~Yeo}\affiliation{\instKISTI} % 2204
  \author{J.~H.~Yin}\affiliation{\instKorea} % 2365
  \author{M.~Yonenaga}\affiliation{\instTokyoMetropolitan} % 2411
  \author{Y.~M.~Yook}\affiliation{\instIHEPChina} % 2453
  \author{T.~Yoshinobu}\affiliation{\instNiigata} % 2429
  \author{C.~Z.~Yuan}\affiliation{\instIHEPChina} % 2088
  \author{G.~Yuan}\affiliation{\instUSTC} % 7243
  \author{W.~Yuan}\affiliation{\instPadovaINFN} % 2504
  \author{Y.~Yusa}\affiliation{\instNiigata} % 2357
  \author{L.~Zani}\affiliation{\instCPPM} % 2529
  \author{J.~Z.~Zhang}\affiliation{\instIHEPChina} % 2349
  \author{Y.~Zhang}\affiliation{\instUSTC} % 2607
  \author{Z.~Zhang}\affiliation{\instUSTC} % 5363
  \author{V.~Zhilich}\affiliation{\instBINP}\affiliation{\instNSU} % 4703
  \author{Q.~D.~Zhou}\affiliation{\instNagoya}\affiliation{\instNagoyaIAR} % 7323
  \author{X.~Y.~Zhou}\affiliation{\instBeihang} % 2380
  \author{V.~I.~Zhukova}\affiliation{\instLPI} % 2387
  \author{V.~Zhulanov}\affiliation{\instBINP}\affiliation{\instNSU} % 4983
  \author{A.~Zupanc}\affiliation{\instLjubljanaJSI} % 2543
\collaboration{Belle II Collaboration}

==> title.tex <==
% WRITE THE TITLE IN THIS FILE
$\tau$ lepton mass measurement at {\belletwo}
